Adaptive coding efficiency in recurrent cortical circuits via gain control

Sensory systems across all modalities and species exhibit adaptation to continuously changing input statistics. Individual neurons have been shown to modulate their response gains so as to maximize information transmission in different stimulus contexts. Experimental measurements have revealed additional, nuanced sensory adaptation effects including changes in response maxima and minima, tuning curve repulsion from the adapter stimulus, and stimulus-driven response decorrelation. Existing explanations of these phenomena rely on changes in inter-neuronal synaptic efficacy, which, while more flexible, are unlikely to operate as rapidly or reversibly as single neuron gain modulations. Using published V1 population adaptation data, we show that propagation of single neuron gain changes in a recurrent network is sufficient to capture the entire set of observed adaptation effects. We propose a novel adaptive efficient coding objective with which single neuron gains are modulated, maximizing the fidelity of the stimulus representation while minimizing overall activity in the network. From this objective, we analytically derive a set of gains that optimize the trade-off between preserving information about the stimulus and conserving metabolic resources. Our model generalizes well-established concepts of single neuron adaptive gain control to recurrent populations, and parsimoniously explains experimental adaptation data.

==> deprecated/cover_letter.tex <==
Dear Editor(s),

We would be grateful if you would consider the attached manuscript, ``Statistical adaptation via gain control in recurrent neural networks", to be considered for publication as an article in [xxxx].

We believe our work is likely to have significant impact on the field of and sensory neuroscience, and is therefore well-suited to a journal such as [xxxx].
An earlier version of this work was presented at Computational \& Systems Neuroscience (CoSyNe) 2022, but has not otherwise been published, and is not under consideration by any other journal.
Suitable reviewers for this project, each with expertise and prior work in statistical adaptation or normative theory, include: Adrienne Fairhall (U. Washington), Xuexin Wei (UT Austin), Wiktor Mlynarski (IST Austria), Ann Hermundstad (Janelia), Adam Kohn (Einstein College), Gabrielle Gutierrez (Columbia).

